Observation of $e^+e^-\to \pi^0\pi^0 h_c$ and a neutral charmoniumlike structure $Z_c(4020)^0$

Using data collected with the BESIII detector operating at the Beijing Electron Positron Collider at center-of-mass energies of $\sqrt{s}=4.23$, 4.26, and 4.36~GeV, we observe $\EE\to \pphc$ for the first time. The Born cross sections are measured and found to be about half of those of $\EE\to \pi^+\pi^-h_c$ within less than 2$\sigma$. In the $\pi^0h_c$ mass spectrum, a structure at 4.02~GeV/$c^2$ is found. It is most likely to be the neutral isospin partner of the $\zcp^{\pm}$ observed in the process of $\EE\to \pi^+\pi^-h_c$ is found. A fit to the $\pi^0 h_c$ invariant mass spectrum, with the width of the $\zcpn$ fixed to that of its charged isospin partner and possible interferences with non-$\zcpn$ amplitudes neglected, gives a mass of ($4023.9\pm 2.2 \pm 3.8$)~MeV/$c^2$ for the $\zcpn$, where the first error is statistical and the second systematic.

==> authors_sep2014.tex <==
\author{
\begin{small}
\begin{center}
M.~Ablikim$^{1}$, M.~N.~Achasov$^{8,a}$, X.~C.~Ai$^{1}$,
      O.~Albayrak$^{4}$, M.~Albrecht$^{3}$, D.~J.~Ambrose$^{42}$,
      A.~Amoroso$^{46A,46C}$, F.~F.~An$^{1}$, Q.~An$^{43}$, J.~Z.~Bai$^{1}$,
      R.~Baldini Ferroli$^{19A}$, Y.~Ban$^{30}$, D.~W.~Bennett$^{18}$,
      J.~V.~Bennett$^{4}$, M.~Bertani$^{19A}$, D.~Bettoni$^{20A}$,
      J.~M.~Bian$^{41}$, F.~Bianchi$^{46A,46C}$, E.~Boger$^{22,g}$,
      O.~Bondarenko$^{24}$, I.~Boyko$^{22}$, R.~A.~Briere$^{4}$,
      H.~Cai$^{48}$, X.~Cai$^{1}$, O. ~Cakir$^{38A}$, A.~Calcaterra$^{19A}$,
      G.~F.~Cao$^{1}$, S.~A.~Cetin$^{38B}$, J.~F.~Chang$^{1}$,
      G.~Chelkov$^{22,b}$, G.~Chen$^{1}$, H.~S.~Chen$^{1}$,
      H.~Y.~Chen$^{2}$, J.~C.~Chen$^{1}$, M.~L.~Chen$^{1}$,
      S.~J.~Chen$^{28}$, X.~Chen$^{1}$, X.~R.~Chen$^{25}$, Y.~B.~Chen$^{1}$,
      H.~P.~Cheng$^{16}$, X.~K.~Chu$^{30}$, Y.~P.~Chu$^{1}$,
      G.~Cibinetto$^{20A}$, D.~Cronin-Hennessy$^{41}$, H.~L.~Dai$^{1}$,
      J.~P.~Dai$^{1}$, D.~Dedovich$^{22}$, Z.~Y.~Deng$^{1}$,
      A.~Denig$^{21}$, I.~Denysenko$^{22}$, M.~Destefanis$^{46A,46C}$,
      F.~De~Mori$^{46A,46C}$, Y.~Ding$^{26}$, C.~Dong$^{29}$, J.~Dong$^{1}$,
      L.~Y.~Dong$^{1}$, M.~Y.~Dong$^{1}$, S.~X.~Du$^{50}$, P.~F.~Duan$^{1}$,
      J.~Z.~Fan$^{37}$, J.~Fang$^{1}$, S.~S.~Fang$^{1}$, X.~Fang$^{43}$,
      Y.~Fang$^{1}$, L.~Fava$^{46B,46C}$, F.~Feldbauer$^{21}$,
      G.~Felici$^{19A}$, C.~Q.~Feng$^{43}$, E.~Fioravanti$^{20A}$,
      C.~D.~Fu$^{1}$, Q.~Gao$^{1}$, Y.~Gao$^{37}$, I.~Garzia$^{20A}$,
      K.~Goetzen$^{9}$, W.~X.~Gong$^{1}$, W.~Gradl$^{21}$,
      M.~Greco$^{46A,46C}$, M.~H.~Gu$^{1}$, Y.~T.~Gu$^{11}$,
      Y.~H.~Guan$^{1}$, A.~Q.~Guo$^{1}$, L.~B.~Guo$^{27}$, T.~Guo$^{27}$,
      Y.~Guo$^{1}$, Y.~P.~Guo$^{21}$, Z.~Haddadi$^{24}$, A.~Hafner$^{21}$,
      S.~Han$^{48}$, Y.~L.~Han$^{1}$, F.~A.~Harris$^{40}$, K.~L.~He$^{1}$,
      Z.~Y.~He$^{29}$, T.~Held$^{3}$, Y.~K.~Heng$^{1}$, Z.~L.~Hou$^{1}$,
      C.~Hu$^{27}$, H.~M.~Hu$^{1}$, J.~F.~Hu$^{46A}$, T.~Hu$^{1}$,
      Y.~Hu$^{1}$, G.~M.~Huang$^{5}$, G.~S.~Huang$^{43}$,
      H.~P.~Huang$^{48}$, J.~S.~Huang$^{14}$, X.~T.~Huang$^{32}$,
      Y.~Huang$^{28}$, T.~Hussain$^{45}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{29}$,
      X.~B.~Ji$^{1}$, X.~L.~Ji$^{1}$, L.~L.~Jiang$^{1}$, L.~W.~Jiang$^{48}$,
      X.~S.~Jiang$^{1}$, J.~B.~Jiao$^{32}$, Z.~Jiao$^{16}$, D.~P.~Jin$^{1}$,
      S.~Jin$^{1}$, T.~Johansson$^{47}$, A.~Julin$^{41}$,
      N.~Kalantar-Nayestanaki$^{24}$, X.~L.~Kang$^{1}$, X.~S.~Kang$^{29}$,
      M.~Kavatsyuk$^{24}$, B.~C.~Ke$^{4}$, R.~Kliemt$^{13}$,
      B.~Kloss$^{21}$, O.~B.~Kolcu$^{38B,c}$, B.~Kopf$^{3}$,
      M.~Kornicer$^{40}$, W.~Kuehn$^{23}$, A.~Kupsc$^{47}$, W.~Lai$^{1}$,
      J.~S.~Lange$^{23}$, M.~Lara$^{18}$, P. ~Larin$^{13}$, M.~Leyhe$^{3}$,
      Cheng~Li$^{43}$, D.~M.~Li$^{50}$, F.~Li$^{1}$, G.~Li$^{1}$,
      H.~B.~Li$^{1}$, J.~C.~Li$^{1}$, Jin~Li$^{31}$, K.~Li$^{12}$,
      K.~Li$^{32}$, Q.~J.~Li$^{1}$, T. ~Li$^{32}$, W.~D.~Li$^{1}$,
      W.~G.~Li$^{1}$, X.~L.~Li$^{32}$, X.~M.~Li$^{11}$, X.~N.~Li$^{1}$,
      X.~Q.~Li$^{29}$, Z.~B.~Li$^{36}$, H.~Liang$^{43}$, Y.~F.~Liang$^{34}$,
      Y.~T.~Liang$^{23}$, G.~R.~Liao$^{10}$, D.~X.~Lin$^{13}$,
      B.~J.~Liu$^{1}$, C.~L.~Liu$^{4}$, C.~X.~Liu$^{1}$, F.~H.~Liu$^{33}$,
      Fang~Liu$^{1}$, Feng~Liu$^{5}$, H.~B.~Liu$^{11}$, H.~H.~Liu$^{1}$,
      H.~H.~Liu$^{15}$, H.~M.~Liu$^{1}$, J.~Liu$^{1}$, J.~P.~Liu$^{48}$,
      J.~Y.~Liu$^{1}$, K.~Liu$^{37}$, K.~Y.~Liu$^{26}$, L.~D.~Liu$^{30}$,
      Q.~Liu$^{39}$, S.~B.~Liu$^{43}$, X.~Liu$^{25}$, X.~X.~Liu$^{39}$,
      Y.~B.~Liu$^{29}$, Z.~A.~Liu$^{1}$, Zhiqiang~Liu$^{1}$,
      Zhiqing~Liu$^{21}$, H.~Loehner$^{24}$, X.~C.~Lou$^{1,d}$,
      H.~J.~Lu$^{16}$, J.~G.~Lu$^{1}$, R.~Q.~Lu$^{17}$, Y.~Lu$^{1}$,
      Y.~P.~Lu$^{1}$, C.~L.~Luo$^{27}$, M.~X.~Luo$^{49}$, T.~Luo$^{40}$,
      X.~L.~Luo$^{1}$, M.~Lv$^{1}$, X.~R.~Lyu$^{39}$, F.~C.~Ma$^{26}$,
      H.~L.~Ma$^{1}$, Q.~M.~Ma$^{1}$, S.~Ma$^{1}$, T.~Ma$^{1}$,
      X.~N.~Ma$^{29}$, X.~Y.~Ma$^{1}$, F.~E.~Maas$^{13}$,
      M.~Maggiora$^{46A,46C}$, Q.~A.~Malik$^{45}$, Y.~J.~Mao$^{30}$,
      Z.~P.~Mao$^{1}$, S.~Marcello$^{46A,46C}$, J.~G.~Messchendorp$^{24}$,
      J.~Min$^{1}$, T.~J.~Min$^{1}$, R.~E.~Mitchell$^{18}$, X.~H.~Mo$^{1}$,
      Y.~J.~Mo$^{5}$, H.~Moeini$^{24}$, C.~Morales Morales$^{13}$, K.~Moriya$^{18}$,
      N.~Yu.~Muchnoi$^{8,a}$, H.~Muramatsu$^{41}$, Y.~Nefedov$^{22}$,
      F.~Nerling$^{13}$, I.~B.~Nikolaev$^{8,a}$, Z.~Ning$^{1}$,
      S.~Nisar$^{7}$, S.~L.~Niu$^{1}$, X.~Y.~Niu$^{1}$, S.~L.~Olsen$^{31}$,
      Q.~Ouyang$^{1}$, S.~Pacetti$^{19B}$, P.~Patteri$^{19A}$,
      M.~Pelizaeus$^{3}$, H.~P.~Peng$^{43}$, K.~Peters$^{9}$,
      J.~L.~Ping$^{27}$, R.~G.~Ping$^{1}$, R.~Poling$^{41}$,
      Y.~N.~Pu$^{17}$, M.~Qi$^{28}$, S.~Qian$^{1}$, C.~F.~Qiao$^{39}$,
      L.~Q.~Qin$^{32}$, N.~Qin$^{48}$, X.~S.~Qin$^{1}$, Y.~Qin$^{30}$,
      Z.~H.~Qin$^{1}$, J.~F.~Qiu$^{1}$, K.~H.~Rashid$^{45}$,
      C.~F.~Redmer$^{21}$, H.~L.~Ren$^{17}$, M.~Ripka$^{21}$, G.~Rong$^{1}$,
      X.~D.~Ruan$^{11}$, V.~Santoro$^{20A}$, A.~Sarantsev$^{22,e}$,
      M.~Savri\'e$^{20B}$, K.~Schoenning$^{47}$, S.~Schumann$^{21}$,
      W.~Shan$^{30}$, M.~Shao$^{43}$, C.~P.~Shen$^{2}$, P.~X.~Shen$^{29}$,
      X.~Y.~Shen$^{1}$, H.~Y.~Sheng$^{1}$, M.~R.~Shepherd$^{18}$,
      W.~M.~Song$^{1}$, X.~Y.~Song$^{1}$, S.~Sosio$^{46A,46C}$,
      S.~Spataro$^{46A,46C}$, B.~Spruck$^{23}$, G.~X.~Sun$^{1}$,
      J.~F.~Sun$^{14}$, S.~S.~Sun$^{1}$, Y.~J.~Sun$^{43}$, Y.~Z.~Sun$^{1}$,
      Z.~J.~Sun$^{1}$, C.~J.~Tang$^{34}$, X.~Tang$^{1}$, I.~Tapan$^{38C}$,
      E.~H.~Thorndike$^{42}$, M.~Tiemens$^{24}$, D.~Toth$^{41}$,
      M.~Ullrich$^{23}$, I.~Uman$^{38B}$, G.~S.~Varner$^{40}$,
      B.~Wang$^{29}$, B.~L.~Wang$^{39}$, D.~Wang$^{30}$, D.~Y.~Wang$^{30}$,
      K.~Wang$^{1}$, L.~L.~Wang$^{1}$, L.~S.~Wang$^{1}$, M.~Wang$^{32}$,
      P.~Wang$^{1}$, P.~L.~Wang$^{1}$, Q.~J.~Wang$^{1}$, S.~G.~Wang$^{30}$,
      W.~Wang$^{1}$, X.~F. ~Wang$^{37}$, Y.~F.~Wang$^{1}$,
      Y.~Q.~Wang$^{21}$, Z.~Wang$^{1}$, Z.~G.~Wang$^{1}$, Z.~H.~Wang$^{43}$,
      Z.~Y.~Wang$^{1}$, D.~H.~Wei$^{10}$, J.~B.~Wei$^{30}$,
      P.~Weidenkaff$^{21}$, S.~P.~Wen$^{1}$, U.~Wiedner$^{3}$,
      M.~Wolke$^{47}$, L.~H.~Wu$^{1}$, Z.~Wu$^{1}$, L.~G.~Xia$^{37}$,
      Y.~Xia$^{17}$, D.~Xiao$^{1}$, Z.~J.~Xiao$^{27}$, Y.~G.~Xie$^{1}$,
      Q.~L.~Xiu$^{1}$, G.~F.~Xu$^{1}$, L.~Xu$^{1}$, Q.~J.~Xu$^{12}$,
      Q.~N.~Xu$^{39}$, X.~P.~Xu$^{35}$, Z.~Xue$^{1}$, L.~Yan$^{43}$,
      W.~B.~Yan$^{43}$, W.~C.~Yan$^{43}$, Y.~H.~Yan$^{17}$,
      H.~X.~Yang$^{1}$, L.~Yang$^{48}$, Y.~Yang$^{5}$, Y.~X.~Yang$^{10}$,
      H.~Ye$^{1}$, M.~Ye$^{1}$, M.~H.~Ye$^{6}$, J.~H.~Yin$^{1}$,
      B.~X.~Yu$^{1}$, C.~X.~Yu$^{29}$, H.~W.~Yu$^{30}$, J.~S.~Yu$^{25}$,
      C.~Z.~Yuan$^{1}$, W.~L.~Yuan$^{28}$, Y.~Yuan$^{1}$,
      A.~Yuncu$^{38B,f}$, A.~A.~Zafar$^{45}$, A.~Zallo$^{19A}$,
      Y.~Zeng$^{17}$, B.~X.~Zhang$^{1}$, B.~Y.~Zhang$^{1}$, C.~Zhang$^{28}$,
      C.~C.~Zhang$^{1}$, D.~H.~Zhang$^{1}$, H.~H.~Zhang$^{36}$,
      H.~T.~Zhang$^{1}$, H.~Y.~Zhang$^{1}$, J.~J.~Zhang$^{1}$,
      J.~L.~Zhang$^{1}$, J.~Q.~Zhang$^{1}$, J.~W.~Zhang$^{1}$,
      J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1}$, K.~Zhang$^{1}$, L.~Zhang$^{1}$,
      S.~H.~Zhang$^{1}$, X.~J.~Zhang$^{1}$, X.~Y.~Zhang$^{32}$,
      Y.~Zhang$^{1}$, Y.~H.~Zhang$^{1}$, Z.~H.~Zhang$^{5}$,
      Z.~P.~Zhang$^{43}$, Z.~Y.~Zhang$^{48}$, G.~Zhao$^{1}$,
      J.~W.~Zhao$^{1}$, J.~Y.~Zhao$^{1}$, J.~Z.~Zhao$^{1}$, Lei~Zhao$^{43}$,
      Ling~Zhao$^{1}$, M.~G.~Zhao$^{29}$, Q.~Zhao$^{1}$, Q.~W.~Zhao$^{1}$,
      S.~J.~Zhao$^{50}$, T.~C.~Zhao$^{1}$, Y.~B.~Zhao$^{1}$,
      Z.~G.~Zhao$^{43}$, A.~Zhemchugov$^{22,g}$, B.~Zheng$^{44}$,
      J.~P.~Zheng$^{1}$, Y.~H.~Zheng$^{39}$, B.~Zhong$^{27}$, L.~Zhou$^{1}$,
      Li~Zhou$^{29}$, X.~Zhou$^{48}$, X.~K.~Zhou$^{43}$, X.~R.~Zhou$^{43}$,
      X.~Y.~Zhou$^{1}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1}$, S.~Zhu$^{1}$,
      X.~L.~Zhu$^{37}$, Y.~C.~Zhu$^{43}$, Y.~S.~Zhu$^{1}$, Z.~A.~Zhu$^{1}$,
      J.~Zhuang$^{1}$, B.~S.~Zou$^{1}$, J.~H.~Zou$^{1}$
      \\
      \vspace{0.2cm}
      (BESIII Collaboration)\\
      \vspace{0.2cm} {\it
        $^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
        $^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
        $^{3}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
        $^{4}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
        $^{5}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
        $^{6}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
        $^{7}$ COMSATS Institute of Information Technology, Lahore, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
        $^{8}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
        $^{9}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
        $^{10}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
        $^{11}$ GuangXi University, Nanning 530004, People's Republic of China\\
        $^{12}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
        $^{13}$ Helmholtz Institute Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
        $^{14}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
        $^{15}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
        $^{16}$ Huangshan College, Huangshan 245000, People's Republic of China\\
        $^{17}$ Hunan University, Changsha 410082, People's Republic of China\\
        $^{18}$ Indiana University, Bloomington, Indiana 47405, USA\\
        $^{19}$ (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN and University of Perugia, I-06100, Perugia, Italy\\
        $^{20}$ (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
        $^{21}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
        $^{22}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
        $^{23}$ Justus Liebig University Giessen, II. Physikalisches
        Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
        $^{24}$ KVI-CART, University of Groningen, NL-9747 AA Groningen, The Netherlands\\
        $^{25}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
        $^{26}$ Liaoning University, Shenyang 110036, People's Republic of China\\
        $^{27}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
        $^{28}$ Nanjing University, Nanjing 210093, People's Republic of China\\
        $^{29}$ Nankai University, Tianjin 300071, People's Republic of China\\
        $^{30}$ Peking University, Beijing 100871, People's Republic of China\\
        $^{31}$ Seoul National University, Seoul, 151-747 Korea\\
        $^{32}$ Shandong University, Jinan 250100, People's Republic of China\\
        $^{33}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
        $^{34}$ Sichuan University, Chengdu 610064, People's Republic of China\\
        $^{35}$ Soochow University, Suzhou 215006, People's Republic of China\\
        $^{36}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
        $^{37}$ Tsinghua University, Beijing 100084, People's Republic of China\\
        $^{38}$ (A)Ankara University, Dogol Caddesi, 06100 Tandogan, Ankara, Turkey; (B)Dogus University, 34722 Istanbul, Turkey; (C)Uludag University, 16059 Bursa, Turkey\\
        $^{39}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
        $^{40}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
        $^{41}$ University of Minnesota, Minneapolis, Minnesota 55455, USA\\
        $^{42}$ University of Rochester, Rochester, New York 14627, USA\\
        $^{43}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
        $^{44}$ University of South China, Hengyang 421001, People's Republic of China\\
        $^{45}$ University of the Punjab, Lahore-54590, Pakistan\\
        $^{46}$ (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
        $^{47}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
        $^{48}$ Wuhan University, Wuhan 430072, People's Republic of China\\
        $^{49}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
        $^{50}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
        \vspace{0.2cm}
        $^{a}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
        $^{b}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia and at the Functional Electronics Laboratory, Tomsk State University, Tomsk, 634050, Russia \\
        $^{c}$ Currently at Istanbul Arel University, Kucukcekmece, Istanbul, Turkey\\
        $^{d}$ Also at University of Texas at Dallas, Richardson, Texas 75083, USA\\
        $^{e}$ Also at the PNPI, Gatchina 188300, Russia\\
        $^{f}$ Also at Bogazici University, 34342 Istanbul, Turkey\\
        $^{g}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\~\\~\\
      }\end{center}
    \vspace{0.4cm}
  \end{small}
}

%\affiliation{}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "pi0pi0hc_prl"
%%% End:

